Chained Tuning Leads to Biased Forgetting

Large language models (LLMs) are often fine-tuned for use on downstream tasks, though this can degrade capabilities learned during previous training. This phenomenon, often referred to as catastrophic forgetting, has important potential implications for the safety of deployed models. In this work, we first show that models trained on downstream tasks forget their safety tuning to a greater extent than models trained in the opposite order. Second, we show that forgetting disproportionately impacts safety information about certain groups. To quantify this phenomenon, we define a new metric we term biased forgetting. We conduct a systematic evaluation of the effects of task ordering on forgetting and apply mitigations that can help the model recover from the forgetting observed. We hope our findings can better inform methods for chaining the finetuning of LLMs in continual learning settings to enable training of safer and less toxic models.

==> tables/ordering_result.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lccccc}
& & & Capability & Safety \\
\toprule
  & $\mathrm{Acc}_{ARC}$ &  $\mathrm{Acc}_{TQA}$ & $\mathrm{Forgetting}_{ARC}$ &  $\mathrm{Forgetting}_{TQA}$  \\ 
\midrule
ARC$\rightarrow$TQA &     77.41   &    90.3     &      -0.03      &       --         \\
TQA$\rightarrow$ARC &     75.15    &  85.74         &      --      &    4.81        \\ 
\midrule
    & $\mathrm{Acc}_{ARC}$ &  $\mathrm{Acc}_{BBQ}$ & $\mathrm{Forgetting}_{ARC}$ &  $\mathrm{Forgetting}_{BBQ}$\\ 
\midrule
ARC$\rightarrow$BBQ &     75.77   &    51.05     &     1.61      &       --        \\
BBQ$\rightarrow$ARC &     74.43    &  47.59         &    --         &   1.92            \\ 
\midrule
    & $\mathrm{Acc}_{ARC}$ &  $\mathrm{Acc}_{SD}$ & $\mathrm{Forgetting}_{ARC}$ &  $\mathrm{Forgetting}_{SD}$\\ 
\midrule
ARC$\rightarrow$SD &     76.83   &    98.10     &     0.68      &       --        \\
SD$\rightarrow$ARC &     75.95    &  94.25         &    --         &   2.83            \\ 
\midrule
  & $\mathrm{Acc}_{CQA2}$ &  $\mathrm{Acc}_{TQA}$ & $\mathrm{Forgetting}_{CQA2}$ &  $\mathrm{Forgetting}_{TQA}$  \\ 
\midrule
CQA2$\rightarrow$TQA &     51.79   &    90.99    &      9.29      &       --         \\
TQA$\rightarrow$CQA2 &     60.60    &   53.11         &      --      &    38.05        \\ 
\midrule
    & $\mathrm{Acc}_{CQA2}$ &  $\mathrm{Acc}_{BBQ}$ & $\mathrm{Forgetting}_{CQA2}$ &  $\mathrm{Forgetting}_{BBQ}$\\ 
\midrule
CQA2$\rightarrow$BBQ &     53.71   &    98.18     &     7.37      &       --        \\
BBQ$\rightarrow$CQA2 &     59.43    &  84.49         &    --         &   13.52           \\ 
\midrule
    & $\mathrm{Acc}_{CQA2}$ &  $\mathrm{Acc}_{SD}$ & $\mathrm{Forgetting}_{CQA2}$ &  $\mathrm{Forgetting}_{SD}$\\ 
\midrule
CQA2$\rightarrow$SD &     76.83   &    98.10     &     0.68      &       --        \\
SD$\rightarrow$CQA2 &     75.95    &  94.25         &    --         &   2.83            \\ 
\midrule
  & $\mathrm{Acc}_{CQA}$ &  $\mathrm{Acc}_{TQA}$ & $\mathrm{Forgetting}_{CQA}$ &  $\mathrm{Forgetting}_{TQA}$  \\ 
\midrule
CQA$\rightarrow$TQA &     77.11   &    90.38    &      -0.05      &       --         \\
TQA$\rightarrow$CQA &     77.04    &   87.18         &      --      &    3.98        \\ 
\midrule
    & $\mathrm{Acc}_{CQA}$ &  $\mathrm{Acc}_{BBQ}$ & $\mathrm{Forgetting}_{CQA}$ &  $\mathrm{Forgetting}_{BBQ}$\\ 
\midrule
CQA$\rightarrow$BBQ &     76.01   &    97.75     &     16.87      &       --        \\
BBQ$\rightarrow$CQA &     77.83    &  51.16         &    --         &   46.85           \\ 
\midrule
    & $\mathrm{Acc}_{CQA}$ &  $\mathrm{Acc}_{SD}$ & $\mathrm{Forgetting}_{CQA}$ &  $\mathrm{Forgetting}_{SD}$\\ 
\midrule
CQA$\rightarrow$SD &        &        &         &       --        \\
SD$\rightarrow$CQA &         &           &    --         &              \\ 
\bottomrule
\end{tabular}
\caption{Task performance (accuracy \%) and forgetting when tuning in different order. Forgetting is measured with respect to the performance change on a task to the first task. In this experiment, we use the same training hyper-parameters for the first and second task (learning rate $1e^{-5}$, and batch size 16). }
% \label{table:ordering_table}
\end{table*}
